A decision support framework for optimal vaccine distribution across a multi-tier cold chain network

In this paper, we present a decision support framework for optimizing multiple aspects of vaccine distribution across a multitier cold chain network. We propose two multi-period optimization formulations within this framework: first to minimize inventory, ordering, transportation, personnel and shortage costs associated with a single vaccine; the second being an extension of the first for the case when multiple vaccines with differing efficacies and costs are available for the same disease. Vaccine transportation and administration lead times are also incorporated within the models. We also develop robust optimization versions of the single vaccine model to account for the impact of uncertainty in model parameters on the optimal vaccine distribution solution. We use the case of the Indian state of Bihar and COVID-19 vaccines to illustrate the implementation of the framework. We present computational experiments to demonstrate: (a) the organization of the model outputs; (b) how the models can be used to assess the impact of cold chain point storage capacities, transportation vehicle capacities, and manufacturer capacities on the optimal vaccine distribution pattern; and (c) the impact of vaccine efficacies and associated costs such as ordering and transportation costs on the vaccine selection decision informed by the model. We then consider the computational expense of the framework for realistic problem instances, and suggest multiple preprocessing techniques to reduce their computational burden. Finally, we also demonstrate how the robust versions of the single vaccine model outperform the deterministic version under multiple levels of uncertainty in key model parameters. Our study presents public health authorities and other stakeholders with a vaccine distribution and capacity planning tool for multi-tier cold chain networks.

==> Formulation/constraints_robust.tex <==
\begin{flushleft}
    \normalsize \textbf{Subject to constraints:}
\end{flushleft}

The constraints follow single commodity problem with the following additional constraints pertaining to budgeted uncertainty:
\begin{itemize}
    \setcounter{equation}{0}
        \item Budgeted uncertainty constraints corresponding to holding costs.
        \begin{equation}
            \alpha_{a}^{h} + \beta_{a}^{h} \geq \sum_{t} I^{a}_{t}~ \delta_{a}^{h} ~~ \forall a ~~ a \in \{g,s,r,d,i\}
        \end{equation}
        For example,
        \begin{equation*}
            \alpha_{g}^{h} + \beta_{g}^{h} \geq \sum_{t} I^{g}_{t}~ \delta_{g}^{h} ~~ \forall g
        \end{equation*}
        % \begin{equation}
        %     \alpha_{s}^{h} + \beta_{s}^{h} \geq \sum_{t} I^{s}_{t}~ \delta_{s}^{h} ~~~~ \forall s
        % \end{equation}
        % \begin{equation}
        %     \alpha_{r}^{h} + \beta_{r}^{h} \geq \sum_{t} I^{r}_{t}~ \delta_{r}^{h} ~~~~ \forall r
        % \end{equation}
        % \begin{equation}
        %     \alpha_{d}^{h} + \beta_{d}^{h} \geq \sum_{t} I^{d}_{t}~ \delta_{d}^{h} ~~~~ \forall d
        % \end{equation}
        % \begin{equation}
        %     \alpha_{i}^{h} + \beta_{i}^{h} \geq \sum_{t} I^{i}_{t}~ \delta_{i}^{h} ~~~~ \forall i
        % \end{equation}
        
        \item Budgeted uncertainty constraints corresponding to ordering costs.
        \begin{equation}
            \alpha_{a}^{S} + \beta_{a}^{S} \geq \sum_{b} \sum_{t} x^{ab}_{t}~ \delta_{a}^{S} ~~ \forall a ~~ \text{if}~ a \in \{m,g,s,r,d\}~ \text{then b:= the next lower-tier value from \{g,s,r,d,i\}}
        \end{equation}
        For example,
        \begin{equation*}
            \alpha_{m}^{S} + \beta_{m}^{S} \geq \sum_{g} \sum_{t} x^{mg}_{t}~ \delta_{m}^{S} ~~ \forall m
        \end{equation*}
        % \begin{equation}
        %     \alpha_{g}^{S} + \beta_{g}^{S} \geq \sum_{s} \sum_{t} x^{gs}_{t}~ \delta_{g}^{S} ~~~~~~ \forall g
        % \end{equation}
        % \begin{equation}
        %     \alpha_{s}^{S} + \beta_{s}^{S} \geq \sum_{r} \sum_{t} x^{sr}_{t}~ \delta_{s}^{S} ~~~~~~ \forall s
        % \end{equation}
        % \begin{equation}
        %     \alpha_{r}^{S} + \beta_{r}^{S} \geq \sum_{d} \sum_{t} x^{rd}_{t}~ \delta_{r}^{S} ~~~~~~ \forall r
        % \end{equation}
        % \begin{equation}
        %     \alpha_{d}^{S} + \beta_{d}^{S} \geq \sum_{i} \sum_{t} x^{di}_{t}~ \delta_{d}^{S} ~~~~~~ \forall d
        % \end{equation}
        
    \end{itemize}


==> Formulation/decision_variables_robust.tex <==
\begin{flushleft}
    \normalsize \textbf{Decision Variables}
\end{flushleft}

As is the case with parameters, the decision variables will follow from the single commodity problem, in addition to which we have the following budgeted uncertainty variables.

\begin{itemize}
\item $\alpha$ dual variable for uncertainty in holding costs at each tier: $\alpha_{g}^{h}$, $\alpha_{s}^{h}$, $\alpha_{r}^{h}$, $\alpha_{d}^{h}$, $\alpha_{i}^{h}$. 
\item $\alpha$ dual variable for uncertainty in ordering costs at each tier: $\alpha_{m}^{S}$, $\alpha_{g}^{S}$, $\alpha_{s}^{S}$, $\alpha_{r}^{S}$, $\alpha_{d}^{S}$. 
\item $\beta$ dual variable for uncertainty in holding costs at each tier: $\beta_{g}^{h}$, $\beta_{s}^{h}$, $\beta_{r}^{h}$, $\beta_{d}^{h}$, $\beta_{i}^{h}$. 
\item $\beta$ dual variable for uncertainty in ordering costs at each tier: $\beta_{m}^{S}$, $\beta_{g}^{S}$, $\beta_{s}^{S}$, $\beta_{r}^{S}$, $\beta_{d}^{S}$. 
%  \item Budgeted Uncertainty: $\alpha$ variables
%     \begin{itemize}
%         \item $\alpha$ variable for uncertainty in holding costs at 'g' \hfill $\alpha_{g}^{h}$
%         \item $\alpha$ variable for uncertainty in holding costs at 's' \hfill $\alpha_{s}^{h}$
%         \item $\alpha$ variable for uncertainty in holding costs at 'r' \hfill $\alpha_{r}^{h}$
%         \item $\alpha$ variable for uncertainty in holding costs at 'd' \hfill $\alpha_{d}^{h}$
%         \item $\alpha$ variable for uncertainty in holding costs at 'i' \hfill $\alpha_{i}^{h}$
%         \item $\alpha$ variable for uncertainty in ordering costs from 'm' \hfill $\alpha_{m}^{S}$
%         \item $\alpha$ variable for uncertainty in ordering costs from 'g' \hfill $\alpha_{g}^{S}$
%         \item $\alpha$ variable for uncertainty in ordering costs from 's' \hfill $\alpha_{s}^{S}$
%         \item $\alpha$ variable for uncertainty in ordering costs from 'r'\hfill $\alpha_{r}^{S}$
%         \item $\alpha$ variable for uncertainty in ordering costs from 'd' \hfill $\alpha_{d}^{S}$
%     \end{itemize}
    
    % \item Budgeted Uncertainty: $\beta$ variables
    % \begin{itemize}
    %     \item $\beta$ variable for uncertainty in holding costs at 'g' \hfill $\beta_{g}^{h}$
    %     \item $\beta$ variable for uncertainty in holding costs at 's' \hfill $\beta_{s}^{h}$
    %     \item $\beta$ variable for uncertainty in holding costs at 'r' \hfill $\beta_{r}^{h}$
    %     \item $\beta$ variable for uncertainty in holding costs at 'd' \hfill $\beta_{d}^{h}$
    %     \item $\beta$ variable for uncertainty in holding costs at 'i' \hfill $\beta_{i}^{h}$
    %     \item $\beta$ variable for uncertainty in ordering costs from 'm' \hfill $\beta_{m}^{S}$
    %     \item $\beta$ variable for uncertainty in ordering costs from 'g' \hfill $\beta_{g}^{S}$
    %     \item $\beta$ variable for uncertainty in ordering costs from 's' \hfill $\beta_{s}^{S}$
    %     \item $\beta$ variable for uncertainty in ordering costs from 'r' \hfill $\beta_{r}^{S}$
    %     \item $\beta$ variable for uncertainty in ordering costs from 'd' \hfill $\beta_{d}^{S}$
    % \end{itemize}
\end{itemize}

==> Formulation/objective_robust.tex <==
\begin{flushleft}
    \normalsize \textbf{Objective Function}
\end{flushleft}
\textbf{Min $J$} = \\*

$\mathop{\sum_{t}\sum_{m}\sum_{g}} K^{mg} n_t^{mg} +
\mathop{\sum_{t}\sum_{g}\sum_{s}} K^{gs} n_t^{gs} +
\mathop{\sum_{t}\sum_{s}\sum_{r}} K^{sr} n_t^{sr} +
\mathop{\sum_{t}\sum_{r}\sum_{d}} K^{rd} n_t^{rd}+ \mathop{\sum_{t}\sum_{d}\sum_{i}} K^{di} n_t^{di} +\\*$

\fbox{Transportation cost * no of trucks from one cold chain point to other}\\*

$\mathop{\sum_{t}\sum_{g} h_t^g I_t^g+ \alpha_{g}^{h} \tau_{g}^{h} + \sum_{g} \beta_{g}^{h}} + \mathop{\sum_{t}\sum_{s} h_t^s I_t^s+ \alpha_{s}^{h} \tau_{s}^{h} + \sum_{s} \beta_{s}^{h}}+ \mathop{\sum_{t}\sum_{r} h_t^r I_t^r+ \alpha_{r}^{h} \tau_{r}^{h} + \sum_{r} \beta_{r}^{h}}+\\*$

$\mathop{\sum_{t}\sum_{d} h_t^d I_t^d+ \alpha_{d}^{h} \tau_{d}^{h} + \sum_{d} \beta_{d}^{h}}+ \mathop{\sum_{t}\sum_{i} h_t^i I_t^i+ \alpha_{i}^{h} \tau_{i}^{h} + \sum_{i} \beta_{i}^{h}}+\\*$

\fbox{Holding cost * Inventory at cold chain points}\\*

$\mathop{\sum_{t}\sum_{i}\sum_{j}} P^{j}_{t} s^{ij}_{t} +
\mathop{\sum_{t}\sum_{i}\sum_{j}} \left(1-\eta \right) p~P^j_{t}~ w^{ij}_{t} \\*$

\fbox{Shortage cost * Shortage of vaccine units at clinic }\\*

$\mathop{\sum_{t}\sum_{i}\sum_{j}} V^j w^{ij}_{t} +\\*$

\fbox{Clinical cost * Consumption of vaccine units at clinic }\\*

$\mathop{\sum_{t}\sum_{m}\sum_{g} S_t^{mg} x_t^{mg}+ \alpha_{m}^{S} \tau_{m}^{S} + \sum_{m} \beta_{m}^{S}} + \mathop{\sum_{t}\sum_{g}\sum_{s} S_t^{gs} x_t^{gs}+ \alpha_{g}^{S} \tau_{g}^{S} + \sum_{g} \beta_{g}^{S}}+ \mathop{\sum_{t}\sum_{s}\sum_{r} S_t^{sr} x_t^{sr}+ \alpha_{s}^{S} \tau_{s}^{S} + \sum_{s} \beta_{s}^{S}}+\\*$

$\mathop{\sum_{t}\sum_{r}\sum_{d} S_t^{rd} x_t^{rd}+ \alpha_{r}^{S} \tau_{r}^{S} + \sum_{r} \beta_{r}^{S}}+ \mathop{\sum_{t}\sum_{d}\sum_{i} S_t^{di} x_t^{di} + \alpha_{d}^{S} \tau_{d}^{S} + \sum_{d} \beta_{d}^{S}}+\\*$

\fbox{Ordering cost (cost incurred if even one vaccine unit is ordered)}\\*

$\mathop{\sum_{t}\sum_{i}} L n^i_t +
\mathop{\sum_{t}\sum_{i}} E h^i_t +
\mathop{\sum_{t}\sum_{i}} F f^i_t$\\

\fbox{Labour costs (Wages, hiring and firing costs)}

==> Formulation/parameters_robust.tex <==
\begin{flushleft}
    \normalsize \textbf{Parameters}
\end{flushleft}

All the parameters that are considered for a single commodity problem will be present in the robust version too. In addition, budgeted uncertainty parameters are introduced for the purpose of incorporating robustness in the model.
\begin{itemize}
  \item Maximum deviation of inventory holding cost at each CCP: $\delta^{h}_{g}$, $\delta^{h}_{s}$, $\delta^{h}_{r}$, $\delta^{h}_{d}$, $\delta^{h}_{i}$. Units: INR/dose/week.
  \item Maximum deviation of fixed cost of ordering vaccine from a CCP by the next lower-tier CCP: $\delta^{S}_{m}$, $\delta^{S}_{g}$, $\delta^{S}_{s}$, $\delta^{S}_{r}$, $\delta^{S}_{d}$. Units: INR/delivery.
  \item Number of inventory holding cost parameters with uncertainty at each tier: $\tau^{h}_{g}$, $\tau^{h}_{s}$, $\tau^{h}_{r}$, $\tau^{h}_{d}$, $\tau^{h}_{i}$. 
  \item Number of ordering cost parameters with uncertainty at each tier: $\tau^{S}_{m}$, $\tau^{S}_{g}$, $\tau^{S}_{s}$, $\tau^{S}_{r}$, $\tau^{S}_{d}$.
%   \begin{itemize}
%           \item Maximum deviation of holding cost at 'g' \hfill $\delta^{h}_{g}$
%           \item Maximum deviation of holding cost at 's' \hfill $\delta^{h}_{s}$
%           \item Maximum deviation of holding cost at 'r' \hfill $\delta^{h}_{r}$
%           \item Maximum deviation of holding cost at 'd' \hfill $\delta^{h}_{d}$
%           \item Maximum deviation of holding cost at 'i' \hfill $\delta^{h}_{i}$
%           \item Maximum deviation of ordering cost from 'm' \hfill $\delta^{S}_{m}$
%           \item Maximum deviation of ordering cost from 'g' \hfill $\delta^{S}_{g}$
%           \item Maximum deviation of ordering cost from 's' \hfill $\delta^{S}_{s}$
%           \item Maximum deviation of ordering cost from 'r' \hfill $\delta^{S}_{r}$
%           \item Maximum deviation of ordering cost from 'd' \hfill $\delta^{S}_{d}$
%     \end{itemize}  
    
    % \item \textbf{Budgeted uncertainty parameters: Number of variables with uncertainty}
  
    %   \begin{itemize}
    %       \item Number of uncertain inventory variables at GMSD level \hfill $\tau^{h}_{g}$
    %       \item Number of uncertain inventory variables at SVS level \hfill $\tau^{h}_{s}$
    %       \item Number of uncertain inventory variables at RVS level \hfill $\tau^{h}_{r}$
    %       \item Number of uncertain inventory variables at DVS level \hfill $\tau^{h}_{d}$
    %       \item Number of uncertain inventory variables at clinics level \hfill $\tau^{h}_{i}$
    %       \item Number of uncertain assignment variables at manufacturer level \hfill $\tau^{S}_{m}$
    %       \item Number of uncertain assignment variables at GMSD level  \hfill $\tau^{S}_{g}$
    %       \item Number of uncertain assignment variables at SVS level \hfill $\tau^{S}_{s}$
    %       \item Number of uncertain assignment variables at RVS level \hfill $\tau^{S}_{r}$
    %       \item Number of uncertain assignment variables at DVS level \hfill $\tau^{S}_{d}$
    %   \end{itemize}
  
\end{itemize}

==> Sections/Mathematical_Formulation_Robust.tex <==
\input{Formulation/robust_methodology}
\input{Formulation/parameters_robust}
% \begin{flushleft}
%     \normalsize \textbf{Total Demand}
% \end{flushleft}
% The following is the total demand by all the sub-groups at all the clinics in the entire planning horizon.\\

% {Q = $\mathop{\sum_{t}^{T}\sum_{i}^{I}\sum_{j}^{J}}$ $d^{ij}_{t}$/w}\\

\input{Formulation/decision_variables_robust}
\input{Formulation/objective_robust}
\input{Formulation/constraints_robust}
